Support matrix machine: A review

Support vector machine (SVM) is one of the most studied paradigms in the realm of machine learning for classification and regression problems. It relies on vectorized input data. However, a significant portion of the real-world data exists in matrix format, which is given as input to SVM by reshaping the matrices into vectors. The process of reshaping disrupts the spatial correlations inherent in the matrix data. Also, converting matrices into vectors results in input data with a high dimensionality, which introduces significant computational complexity. To overcome these issues in classifying matrix input data, support matrix machine (SMM) is proposed. It represents one of the emerging methodologies tailored for handling matrix input data. The SMM method preserves the structural information of the matrix data by using the spectral elastic net property which is a combination of the nuclear norm and Frobenius norm. This article provides the first in-depth analysis of the development of the SMM model, which can be used as a thorough summary by both novices and experts. We discuss numerous SMM variants, such as robust, sparse, class imbalance, and multi-class classification models. We also analyze the applications of the SMM model and conclude the article by outlining potential future research avenues and possibilities that may motivate academics to advance the SMM algorithm.

==> refs.tex <==
@article{xu2015projection,
  title={Projection twin {SMMs} for 2d image data classification},
  author={Xu, Haitao and Fan, Liya and Gao, Xizhan},
  journal={Neural Computing and Applications},
  volume={26},
  pages={91--100},
  year={2015},
  publisher={Springer}
}

@article{zheng2018robust,
  title={Robust support matrix machine for single trial {EEG} classification},
  author={Zheng, Qingqing and Zhu, Fengyuan and Heng, Pheng-Ann},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={26},
  number={3},
  pages={551--562},
  year={2018},
  publisher={IEEE}
}
@article{gaoa2015improved,
  title={IMPROVED LEAST SQUARES TWIN SUPPORT MATRIX MACHINES},
  author={Gaoa, Xizhan and Fanb, Liya and Xub, Haitao},
  year={2015}
}
@article{jiang2018multiple,
  title={Multiple rank multi-linear twin support matrix classification machine},
  author={Jiang, Rong and Yang, Zhi-Xia},
  journal={Journal of Intelligent \& Fuzzy Systems},
  volume={35},
  number={5},
  pages={5741--5754},
  year={2018},
  publisher={IOS Press}
}
@article{dornhege2004boosting,
  title={Boosting bit rates in noninvasive {EEG} single-trial classifications by feature combination and multiclass paradigms},
  author={Dornhege, Guido and Blankertz, Benjamin and Curio, Gabriel and Muller, K-R},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={51},
  number={6},
  pages={993--1002},
  year={2004},
  publisher={IEEE}
}
@article{leeb2007brain,
  title={Brain--computer communication: motivation, aim, and impact of exploring a virtual apartment},
  author={Leeb, Robert and Lee, Felix and Keinrath, Claudia and Scherer, Reinhold and Bischof, Horst and Pfurtscheller, Gert},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={15},
  number={4},
  pages={473--482},
  year={2007},
  publisher={IEEE}
}
@article{pan2022twin,
  title={Twin robust matrix machine for intelligent fault identification of outlier samples in roller bearing},
  author={Pan, Haiyang and Xu, Haifeng and Zheng, Jinde and Tong, Jinyu and Cheng, Jian},
  journal={Knowledge-Based Systems},
  volume={252},
  pages={109391},
  year={2022},
  publisher={Elsevier}
}
@article{pan2022multi,
  title={Multi-class fuzzy support matrix machine for classification in roller bearing fault diagnosis},
  author={Pan, Haiyang and Xu, Haifeng and Zheng, Jinde and Su, Jin and Tong, Jinyu},
  journal={Advanced Engineering Informatics},
  volume={51},
  pages={101445},
  year={2022},
  publisher={Elsevier}
}
@article{ye2019nonlinear,
  title={A nonlinear kernel support matrix machine for matrix learning},
  author={Ye, Yunfei},
  journal={International Journal of Machine Learning and Cybernetics},
  volume={10},
  number={10},
  pages={2725--2738},
  year={2019},
  publisher={Springer}
}
@article{xu2014knn,
  title={{KNN}-based weighted rough $\nu$-twin support vector machine},
  author={Xu, Yitian and Yu, Jia and Zhang, Yuqun},
  journal={Knowledge-Based Systems},
  volume={71},
  pages={303--313},
  year={2014},
  publisher={Elsevier}
}
@article{maboudou2019wavelet,
  title={Wavelet Kernels for Support Matrix Machines},
  author={Maboudou-Tchao, Edgard M},
  journal={Modern Statistical Methods for Spatial and Multivariate Data},
  pages={75--93},
  year={2019},
  publisher={Springer}
}
@article{wenjingXiabilevel2016 ,
  title={LEAST SQUARES SUPPORT MATRIX MACHINES 
BASED ON BILEVEL PROGRAMMING},
  author={Wenjing Xia and Liya Fan},
  journal={International Journal of Applied Mathematics and Machine Learning (IJAMML)},
  pages={1--18},
  year={2016},
  publisher={Springer}
}
@article{mangasarian1999successive,
  title={Successive overrelaxation for support vector machines},
  author={Mangasarian, Olvi L and Musicant, David R},
  journal={IEEE Transactions on Neural Networks},
  volume={10},
  number={5},
  pages={1032--1037},
  year={1999},
  publisher={IEEE}
}
@article{harrow2009quantum,
  title={Quantum algorithm for linear systems of equations},
  author={Harrow, Aram W and Hassidim, Avinatan and Lloyd, Seth},
  journal={Physical Review Letters},
  volume={103},
  number={15},
  pages={150502},
  year={2009},
  publisher={APS}
}
@article{joachims1999svmlight,
  title={Svmlight: Support vector machine},
  author={Joachims, Thorsten},
  journal={SVM-Light Support Vector Machine http://svmlight. joachims. org/, University of Dortmund},
  volume={19},
  number={4},
  pages={25},
  year={1999}
}
@inproceedings{razzak2020cooperative,
  title={Cooperative evolution multiclass support matrix machines},
  author={Razzak, Imran},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}
@article{li2020non,
  title={Non-parallel least squares support matrix machine for rolling bearing fault diagnosis},
  author={Li, Xin and Yang, Yu and Pan, Haiyang and Cheng, Jian and Cheng, Junsheng},
  journal={Mechanism and Machine Theory},
  volume={145},
  pages={103676},
  year={2020},
  publisher={Elsevier}
}
@article{duan2017quantum,
  title={Quantum algorithm for support matrix machines},
  author={Duan, Bojia and Yuan, Jiabin and Liu, Ying and Li, Dan},
  journal={Physical Review A},
  volume={96},
  number={3},
  pages={032301},
  year={2017},
  publisher={APS}
}
@inproceedings{weston2006inference,
  title={Inference with the universum},
  author={Weston, Jason and Collobert, Ronan and Sinz, Fabian and Bottou, L{\'e}on and Vapnik, Vladimir},
  booktitle={Proceedings of the 23rd International Conference on Machine Learning},
  pages={1009--1016},
  year={2006}
}
@article{zheng2018sparse,
  title={Sparse support matrix machine},
  author={Zheng, Qingqing and Zhu, Fengyuan and Qin, Jing and Chen, Badong and Heng, Pheng-Ann},
  journal={Pattern Recognition},
  volume={76},
  pages={715--726},
  year={2018},
  publisher={Elsevier}
}

@ARTICLE{9953061,
  author={Liang, Shuang and Hang, Wenlong and Lei, Baiying and Wang, Jun and Qin, Jing and Choi, Kup-Sze and Zhang, Yu},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={Adaptive Multimodel Knowledge Transfer Matrix Machine for {EEG} Classification}, 
  year={2022},
  volume={},
  number={},
  pages={1-14}}

@inproceedings{dalal2005histograms,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={2005 IEEE computer Society Conference on Computer Vision and Pattern Recognition (CVPR'05)},
  volume={1},
  pages={886--893},
  year={2005},
  organization={Ieee}
}

@inproceedings{fergus2003object,
  title={Object class recognition by unsupervised scale-invariant learning},
  author={Fergus, Robert and Perona, Pietro and Zisserman, Andrew},
  booktitle={2003 IEEE Computer Society Conference on Computer Vision and Pattern Recognition, 2003. Proceedings.},
  volume={2},
  pages={II--II},
  year={2003},
  organization={IEEE}
}
@article{ang2012filter,
  title={Filter bank common spatial pattern algorithm on {BCI} competition IV datasets 2a and 2b},
  author={Ang, Kai Keng and Chin, Zheng Yang and Wang, Chuanchu and Guan, Cuntai and Zhang, Haihong},
  journal={Frontiers in Neuroscience},
  volume={6},
  pages={39},
  year={2012},
  publisher={Frontiers Research Foundation}
}
@article{gu2021ramp,
  title={Ramp sparse support matrix machine and its application in roller bearing fault diagnosis},
  author={Gu, Mingen and Zheng, Jinde and Pan, Haiyang and Tong, Jinyu},
  journal={Applied Soft Computing},
  volume={113},
  pages={107928},
  year={2021},
  publisher={Elsevier}
}


@article{li2021symplectic,
  title={Symplectic weighted sparse support matrix machine for gear fault diagnosis},
  author={Li, Xin and Yang, Yu and Shao, Haidong and Zhong, Xiang and Cheng, Jian and Cheng, Junsheng},
  journal={Measurement},
  volume={168},
  pages={108392},
  year={2021},
  publisher={Elsevier}
}

@article{hang2023deep,
  title={Deep stacked least square support matrix machine with adaptive multi-layer transfer for {EEG} classification},
  author={Hang, Wenlong and Li, Zengguang and Yin, Mingbo and Liang, Shuang and Shen, Hang and Wang, Qiong and Qin, Jin and Choi, Kup-Sze},
  journal={Biomedical Signal Processing and Control},
  volume={82},
  pages={104579},
  year={2023},
  publisher={Elsevier}
}

@article{hang2020deep,
  title={Deep stacked support matrix machine-based representation learning for motor imagery {EEG} classification},
  author={Hang, Wenlong and Feng, Wei and Liang, Shuang and Wang, Qiong and Liu, Xuejun and Choi, Kup-Sze},
  journal={Computer Methods and Programs in Biomedicine},
  volume={193},
  pages={105466},
  year={2020},
  publisher={Elsevier}
}

@article{pan2020symplectic,
  title={Symplectic interactive support matrix machine and its application in roller bearing condition monitoring},
  author={Pan, Haiyang and Yang, Yu and Zheng, Jinde and Li, Xin and Cheng, Junsheng},
  journal={Neurocomputing},
  volume={398},
  pages={1--10},
  year={2020},
  publisher={Elsevier}
}

@article{pan2022pinball,
  title={Pinball transfer support matrix machine for roller bearing fault diagnosis under limited annotation data},
  author={Pan, Haiyang and Sheng, Li and Xu, Haifeng and Tong, Jinyu and Zheng, Jinde and Liu, Qingyun},
  journal={Applied Soft Computing},
  volume={125},
  pages={109209},
  year={2022},
  publisher={Elsevier}
}
@article{zhang2021improved,
  title={An improved quantum algorithm for support matrix machines},
  author={Zhang, Yanbing and Song, Tingting and Wu, Zhihao},
  journal={Quantum Information Processing},
  volume={20},
  pages={1--12},
  year={2021},
  publisher={Springer}
}

@article{li2022auto,
  title={The auto-correlation function aided sparse support matrix machine for {EEG}-based fatigue detection},
  author={Li, Yuxiang and Wang, Dongqing and Liu, Feng},
  journal={IEEE Transactions on Circuits and Systems II: Express Briefs},
  year={2022},
  publisher={IEEE}
}

@article{zheng2017multimodal,
  title={A multimodal approach to estimating vigilance using {EEG} and forehead EOG},
  author={Zheng, Wei-Long and Lu, Bao-Liang},
  journal={Journal of Neural Engineering},
  volume={14},
  number={2},
  pages={026017},
  year={2017},
  publisher={iOP Publishing}
}
@article{zhang2022proximal,
  title={Proximal Support Matrix Machine},
  author={Zhang, Wan and Liu, Yulan},
  journal={Journal of Applied Mathematics and Physics},
  volume={10},
  number={7},
  pages={2268--2291},
  year={2022},
  publisher={Scientific Research Publishing}
}
@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
@inproceedings{nazir2010feature,
  title={Feature selection for efficient gender classification},
  author={Nazir, M and Ishtiaq, Muhammad and Batool, Anab and Jaffar, M Arfan and Mirza, Anwar M},
  booktitle={Proceedings of the 11th WSEAS International Conference},
  pages={70--75},
  year={2010}
}
@inproceedings{lyons1998coding,
  title={Coding facial expressions with gabor wavelets},
  author={Lyons, Michael and Akamatsu, Shigeru and Kamachi, Miyuki and Gyoba, Jiro},
  booktitle={Proceedings Third IEEE International Conference on Automatic Face and Gesture Recognition},
  pages={200--205},
  year={1998},
  organization={IEEE}
}
@inproceedings{luo2015support,
  title={Support matrix machines},
  author={Luo, Luo and Xie, Yubo and Zhang, Zhihua and Li, Wu-Jun},
  booktitle={International Conference on Machine Learning},
  pages={938--947},
  year={2015},
  organization={PMLR}
}

@article{qian2019robust,
  title={Robust multicategory support matrix machines},
  author={Qian, Chengde and Tran-Dinh, Quoc and Fu, Sheng and Zou, Changliang and Liu, Yufeng},
  journal={Mathematical Programming},
  volume={176},
  pages={429--463},
  year={2019},
  publisher={Springer}
}

@inproceedings{altun2010human,
  title={Human activity recognition using inertial/magnetic sensor units},
  author={Altun, Kerem and Barshan, Billur},
  booktitle={Human Behavior Understanding: First International Workshop, HBU 2010, Istanbul, Turkey, August 22, 2010. Proceedings 1},
  pages={38--51},
  year={2010},
  organization={Springer}
}
@article{wang2022sparse,
  title={Sparse norm matrix machine and its application in roller bearing fault diagnosis},
  author={Wang, Meng and Xu, Haifeng and Pan, Haiyang and Xie, Nenggang and Zheng, Jinde},
  journal={Measurement Science and Technology},
  volume={33},
  number={11},
  pages={115114},
  year={2022},
  publisher={IOP Publishing}
}
@article{li2022highly,
  title={Highly efficient fault diagnosis of rotating machinery under time-varying speeds using {LSISMM} and small infrared thermal images},
  author={Li, Xin and Shao, Haidong and Lu, Siliang and Xiang, Jiawei and Cai, Baoping},
  journal={IEEE Transactions on Systems, Man, and Cybernetics: Systems},
  volume={52},
  number={12},
  pages={7328--7340},
  year={2022},
  publisher={IEEE}
}
@article{xu2022dynamic,
  title={Dynamic penalty adaptive matrix machine for the intelligent detection of unbalanced faults in roller bearing},
  author={Xu, Haifeng and Pan, Haiyang and Zheng, Jinde and Liu, Qingyun and Tong, Jinyu},
  journal={Knowledge-Based Systems},
  volume={247},
  pages={108779},
  year={2022},
  publisher={Elsevier}
}

@article{zheng2018multiclass,
  title={Multiclass support matrix machine for single-trial {EEG} classification},
  author={Zheng, Qingqing and Zhu, Fengyuan and Qin, Jing and Heng, Pheng-Ann},
  journal={Neurocomputing},
  volume={275},
  pages={869--880},
  year={2018},
  publisher={Elsevier}
}
@article{razzak2019multiclass,
  title={Multiclass support matrix machines by maximizing the inter-class margin for single trial {EEG} classification},
  author={Razzak, Imran and Blumenstein, Michael and Xu, Guandong},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={27},
  number={6},
  pages={1117--1127},
  year={2019},
  publisher={IEEE}
}

@inproceedings{zhu2017entropy,
  title={Entropy-Based Support Matrix Machine},
  author={Zhu, Changming},
  booktitle={Intelligence Science I: Second IFIP TC 12 International Conference, ICIS 2017, Shanghai, China, October 25-28, 2017, Proceedings 2},
  pages={200--211},
  year={2017},
  organization={Springer}
}
@article{yuan2021support,
  title={Support matrix regression for learning power flow in distribution grid with unobservability},
  author={Yuan, Jingyi and Weng, Yang},
  journal={IEEE Transactions on Power Systems},
  volume={37},
  number={2},
  pages={1151--1161},
  year={2021},
  publisher={IEEE}
}
@article{liao2018urban,
  title={Urban {MV} and {LV} distribution grid topology estimation via group lasso},
  author={Liao, Yizheng and Weng, Yang and Liu, Guangyi and Rajagopal, Ram},
  journal={IEEE Transactions on Power Systems},
  volume={34},
  number={1},
  pages={12--27},
  year={2018},
  publisher={IEEE}
}
@article{osti_1171386,
title = {High Penetration of Photovoltaic Generation Study – Flagstaff Community Power (Final Technical Report, Results of Phases 2-5)},
author = {Narang, David and Ayyanar, Raja and Gemin, Paul and Baggu, Murali and Srinivasan, Devarajan},
doi = {10.2172/1171386},
url = {https://www.osti.gov/biblio/1171386}, journal = {},
place = {United States},
year = {2015},
month = {2}
}

@article{ye2019multi,
  title={Multi-distance support matrix machines},
  author={Ye, Yunfei and Han, Dong},
  journal={Pattern Recognition Letters},
  volume={128},
  pages={237--243},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{lyons1998japanese,
  title={The Japanese female facial expression {(JAFFE)} database},
  author={Lyons, Michael J and Akamatsu, Shigeru and Kamachi, Miyuki and Gyoba, Jiro and Budynek, Julien},
  booktitle={Proceedings of Third International Conference on Automatic Face and Gesture Recognition},
  pages={14--16},
  year={1998}
}
@inproceedings{von1996robust,
  title={Robust classification of hand postures against complex background},
  author={von der Malsburg, C},
  booktitle={Proceedings of the Second International Workshop on Automatic Face and Gesture Recognition, Vermont},
  pages={170--175},
  year={1996}
}

@article{nene1996columbia,
  title={Columbia object image library (coil-20)},
  author={Nene, Sameer A and Nayar, Shree K and Murase, Hiroshi and others},
  year={1996},
  publisher={Citeseer}
}

@article{liang2022adaptive,
  title={Adaptive Multimodel Knowledge Transfer Matrix Machine for {EEG} Classification},
  author={Liang, Shuang and Hang, Wenlong and Lei, Baiying and Wang, Jun and Qin, Jing and Choi, Kup-Sze and Zhang, Yu},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}


@article{razzak2019robust,
  title={Robust sparse representation and multiclass support matrix machines for the classification of motor imagery {EEG} signals},
  author={Razzak, Imran and Hameed, Ibrahim A and Xu, Guandong},
  journal={IEEE Journal of Translational Engineering in Health and Medicine},
  volume={7},
  pages={1--8},
  year={2019},
  publisher={IEEE}
}
@article{pan2019fault,
  title={A fault diagnosis approach for roller bearing based on symplectic geometry matrix machine},
  author={Pan, Haiyang and Yang, Yu and Zheng, Jinde and Li, Xin and Cheng, Junsheng},
  journal={Mechanism and Machine Theory},
  volume={140},
  pages={31--43},
  year={2019},
  publisher={Elsevier}
}
@article{li2021fusion,
  title={A fusion {CWSMM}-based framework for rotating machinery fault diagnosis under strong interference and imbalanced case},
  author={Li, Xin and Cheng, Jian and Shao, Haidong and Liu, Kan and Cai, Baoping},
  journal={IEEE Transactions on Industrial Informatics},
  volume={18},
  number={8},
  pages={5180--5189},
  year={2021},
  publisher={IEEE}
}

@article{zheng2020fault,
  title={A fault classification method for rolling bearing based on multisynchrosqueezing transform and {WOA-SMM}},
  author={Zheng, Jinde and Gu, Mingen and Pan, Haiyang and Tong, Jinyu},
  journal={IEEE Access},
  volume={8},
  pages={215355--215364},
  year={2020},
  publisher={IEEE}
}

@article{pan2022novel,
  title={A novel symplectic relevance matrix machine method for intelligent fault diagnosis of roller bearing},
  author={Pan, Haiyang and Xu, Haifeng and Zheng, Jinde},
  journal={Expert Systems with Applications},
  volume={192},
  pages={116400},
  year={2022},
  publisher={Elsevier}
}

@article{pan2021intelligent,
  title={An intelligent fault diagnosis method for roller bearing using symplectic hyperdisk matrix machine},
  author={Pan, Haiyang and Zheng, Jinde},
  journal={Applied Soft Computing},
  volume={105},
  pages={107284},
  year={2021},
  publisher={Elsevier}
}
@article{pan2022intelligent,
  title={An intelligent fault diagnosis method for roller bearings using an adaptive interactive deviation matrix machine},
  author={Pan, Haiyang and Xu, Haifeng and Zheng, Jinde and Liu, Qingyun and Tong, Jinyu},
  journal={Measurement Science and Technology},
  volume={33},
  number={7},
  pages={075103},
  year={2022},
  publisher={IOP Publishing}
}

@article{pan2023deep,
  title={Deep stacked pinball transfer matrix machine with its application in roller bearing fault diagnosis},
  author={Pan, Haiyang and Sheng, Li and Xu, Haifeng and Zheng, Jinde and Tong, Jinyu and Niu, Limin},
  journal={Engineering Applications of Artificial Intelligence},
  volume={121},
  pages={105991},
  year={2023},
  publisher={Elsevier}
}
@article{gao2016novel,
  title={A novel method for classification of matrix data using twin multiple rank {SMM}s},
  author={Gao, Xizhan and Fan, Liya and Xu, Haitao},
  journal={Applied Soft Computing},
  volume={48},
  pages={546--562},
  year={2016},
  publisher={Elsevier}
}
@article{chen2020novel,
  title={A novel transfer support matrix machine for motor imagery-based brain computer interface},
  author={Chen, Yan and Hang, Wenlong and Liang, Shuang and Liu, Xuejun and Li, Guanglin and Wang, Qiong and Qin, Jing and Choi, Kup-Sze},
  journal={Frontiers in Neuroscience},
  volume={14},
  pages={606949},
  year={2020},
  publisher={Frontiers Media SA}
}
@article{lei2019walking,
  title={Walking imagery evaluation in brain computer interfaces via a multi-view multi-level deep polynomial network},
  author={Lei, Baiying and Liu, Xiaolu and Liang, Shuang and Hang, Wenlong and Wang, Qiong and Choi, Kup-Sze and Qin, Jing},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={27},
  number={3},
  pages={497--506},
  year={2019},
  publisher={IEEE}
}
@inproceedings{tao2005supervised,
  title={Supervised tensor learning},
  author={Tao, Dacheng and Li, Xuelong and Hu, Weiming and Maybank, Stephen and Wu, Xindong},
  booktitle={Fifth IEEE International Conference on Data Mining (ICDM'05)},
  pages={8--pp},
  year={2005},
  organization={IEEE}
}
@article{cai2006support,
  title={Support tensor machines for text categorization},
  author={Cai, Deng and He, Xiaofei and Wen, Ji-Rong and Han, Jiawei and Ma, Wei-Ying},
  year={2006}
}
@article{ye2017matrix,
  title={The Matrix Hilbert space and its application to matrix learning},
  author={Ye, Yunfei},
  journal={arXiv preprint arXiv:1706.08110},
  year={2017}
}
@article{platt1999fast,
  title={Fast training of support vector machines using sequential minimal optimization, advances in kernel methods},
  author={Platt, John C},
  journal={Support Vector Learning},
  pages={185--208},
  year={1999},
  publisher={MIT press}
}
@inproceedings{fung2001proximal,
  title={Proximal support vector machine classifiers},
  author={Fung, Glenn and Mangasarian, Olvi L},
  booktitle={Proceedings of the Seventh ACM SIGKDD International Conference on Knowledge Discovery and Data mining},
  pages={77--86},
  year={2001}
}
@article{chen2011recursive,
  title={Recursive projection twin support vector machine via within-class variance minimization},
  author={Chen, Xiaobo and Yang, Jian and Ye, Qiaolin and Liang, Jun},
  journal={Pattern Recognition},
  volume={44},
  number={10-11},
  pages={2643--2655},
  year={2011},
  publisher={Elsevier}
}
@article{shao2013regularization,
  title={A regularization for the projection twin support vector machine},
  author={Shao, Yuan-Hai and Wang, Zhen and Chen, Wei-Jie and Deng, Nai-Yang},
  journal={Knowledge-Based Systems},
  volume={37},
  pages={203--210},
  year={2013},
  publisher={Elsevier}
}
@inproceedings{kotsia2011support,
  title={Support tucker machines},
  author={Kotsia, Irene and Patras, Ioannis},
  booktitle={CVPR 2011},
  pages={633--640},
  year={2011},
  organization={IEEE}
}
@article{hou2014multiple,
  title={Multiple rank multi-linear {SVM} for matrix data classification},
  author={Hou, Chenping and Nie, Feiping and Zhang, Changshui and Yi, Dongyun and Wu, Yi},
  journal={Pattern Recognition},
  volume={47},
  number={1},
  pages={454--469},
  year={2014},
  publisher={Elsevier}
}
@article{khemchandani2007twin,
  title={Twin support vector machines for pattern classification},
  author={Khemchandani, Reshma and Chandra, Suresh and others},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={29},
  number={5},
  pages={905--910},
  year={2007},
  publisher={IEEE}
}
@article{zhang2021prediction,
  title={Prediction of disease-associated circ{RNA}s via circ{RNA}--disease pair graph and weighted nuclear norm minimization},
  author={Zhang, Yuchen and Lei, Xiujuan and Pan, Yi and Pedrycz, Witold},
  journal={Knowledge-Based Systems},
  volume={214},
  pages={106694},
  year={2021},
  publisher={Elsevier}
}
@article{liu2019saliency,
  title={Saliency detection via double nuclear norm maximization and ensemble manifold regularization},
  author={Liu, Bing and Zhou, Yong and Liu, Peng and Sun, Wei and Li, Shuang and Fang, Xinqiu},
  journal={Knowledge-Based Systems},
  volume={183},
  pages={104850},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{jia2016adaptive,
  title={Adaptive regularizer learning for low rank approximation with application to image denoising},
  author={Jia, Xixi and Feng, Xiangchu and Wang, Weiwei},
  booktitle={2016 IEEE International Conference on Image Processing (ICIP)},
  pages={3096--3100},
  year={2016},
  organization={IEEE}
}
@article{pan2023non,
  title={Non-parallel bounded support matrix machine and its application in roller bearing fault diagnosis},
  author={Pan, Haiyang and Xu, Haifeng and Zheng, Jinde and Tong, Jinyu},
  journal={Information Sciences},
  year={2023},
  publisher={Elsevier}
}
@article{wolpert1992stacked,
  title={Stacked generalization},
  author={Wolpert, David H},
  journal={Neural Networks},
  volume={5},
  number={2},
  pages={241--259},
  year={1992},
  publisher={Elsevier}
}
@article{breiman1996stacked,
  title={Stacked regressions},
  author={Breiman, Leo},
  journal={Machine Learning},
  volume={24},
  pages={49--64},
  year={1996},
  publisher={Springer}
}
@article{vinyals2012learning,
  title={Learning with recursive perceptual representations},
  author={Vinyals, Oriol and Jia, Yangqing and Deng, Li and Darrell, Trevor},
  journal={Advances in Neural Information Processing Systems},
  volume={25},
  year={2012}
}
@article{huang2013support,
  title={Support vector machine classifier with pinball loss},
  author={Huang, Xiaolin and Shi, Lei and Suykens, Johan AK},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={36},
  number={5},
  pages={984--997},
  year={2013},
  publisher={IEEE}
}

@article{tyagi2012review,
  title={A review of {EEG} sensors used for data acquisition},
  author={Tyagi, Aruna and Semwal, Sunil and Shah, Gautam},
  journal={Journal of Computer Applications (IJCA)},
  pages={13--17},
  year={2012}
}
@article{liang2022deep,
  title={Deep {EEG} feature learning via stacking common spatial pattern and support matrix machine},
  author={Liang, Shuang and Hang, Wenlong and Yin, Mingbo and Shen, Hang and Wang, Qiong and Qin, Jin and Choi, Kup-Sze and Zhang, Yu},
  journal={Biomedical Signal Processing and Control},
  volume={74},
  pages={103531},
  year={2022},
  publisher={Elsevier}
}

@article{ramoser2000optimal,
  title={Optimal spatial filtering of single trial {EEG} during imagined hand movement},
  author={Ramoser, Herbert and Muller-Gerking, Johannes and Pfurtscheller, Gert},
  journal={IEEE Transactions on Rehabilitation Engineering},
  volume={8},
  number={4},
  pages={441--446},
  year={2000},
  publisher={IEEE}
}
@article{lotte2007review,
  title={A review of classification algorithms for {EEG}-based brain--computer interfaces},
  author={Lotte, Fabien and Congedo, Marco and L{\'e}cuyer, Anatole and Lamarche, Fabrice and Arnaldi, Bruno},
  journal={Journal of Neural Engineering},
  volume={4},
  number={2},
  pages={R1},
  year={2007},
  publisher={IOP Publishing}
}
@article{cortes1995support,
  title={Support-vector networks},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={Machine Learning},
  volume={20},
  pages={273--297},
  year={1995},
  publisher={Springer}
}
@article{chuang2007fuzzy,
  title={Fuzzy weighted support vector regression with a fuzzy partition},
  author={Chuang, Chen-Chia},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
  volume={37},
  number={3},
  pages={630--640},
  year={2007},
  publisher={IEEE}
}
@article{wang2005new,
  title={A new fuzzy support vector machine to evaluate credit risk},
  author={Wang, Yongqiao and Wang, Shouyang and Lai, Kin Keung},
  journal={IEEE Transactions on Fuzzy Systems},
  volume={13},
  number={6},
  pages={820--831},
  year={2005},
  publisher={IEEE}
}
@article{zhu2016efficient,
  title={Efficient and privacy-preserving online medical prediagnosis framework using nonlinear {SVM}},
  author={Zhu, Hui and Liu, Xiaoxia and Lu, Rongxing and Li, Hui},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={21},
  number={3},
  pages={838--850},
  year={2016},
  publisher={IEEE}
}
@article{zhang2008text,
  title={Text classification based on multi-word with support vector machine},
  author={Zhang, Wen and Yoshida, Taketoshi and Tang, Xijin},
  journal={Knowledge-Based Systems},
  volume={21},
  number={8},
  pages={879--886},
  year={2008},
  publisher={Elsevier}
}
@book{deng2012support,
  title={Support vector machines: optimization based theory, algorithms, and extensions},
  author={Deng, Naiyang and Tian, Yingjie and Zhang, Chunhua},
  year={2012},
  publisher={CRC press}
}
@inproceedings{wolf2007modeling,
  title={Modeling appearances with low-rank {SVM}},
  author={Wolf, Lior and Jhuang, Hueihan and Hazan, Tamir},
  booktitle={2007 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1--6},
  year={2007},
  organization={IEEE}
}
@article{zhou2014regularized,
  title={Regularized matrix regression},
  author={Zhou, Hua and Li, Lexin},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={76},
  number={2},
  pages={463--483},
  year={2014},
  publisher={Oxford University Press}
}

@article{pirsiavash2009bilinear,
  title={Bilinear classifiers for visual recognition},
  author={Pirsiavash, Hamed and Ramanan, Deva and Fowlkes, Charless},
  journal={Advances in Neural Information Processing Systems},
  volume={22},
  year={2009}
}
@inproceedings{srebro2005rank,
  title={Rank, trace-norm and max-norm},
  author={Srebro, Nathan and Shraibman, Adi},
  booktitle={International Conference on Computational Learning Theory},
  pages={545--560},
  year={2005},
  organization={Springer}
}
@inproceedings{huang2013robust,
  title={Robust discrete matrix completion},
  author={Huang, Jin and Nie, Feiping and Huang, Heng},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={27},
  number={1},
  pages={424--430},
  year={2013}
}
@article{candes2012exact,
  title={Exact matrix completion via convex optimization},
  author={Candes, Emmanuel and Recht, Benjamin},
  journal={Communications of the ACM},
  volume={55},
  number={6},
  pages={111--119},
  year={2012},
  publisher={ACM New York, NY, USA}
}
@inproceedings{kobayashi2012efficient,
  title={Efficient optimization for low-rank integrated bilinear classifiers},
  author={Kobayashi, Takumi and Otsu, Nobuyuki},
  booktitle={Computer Vision--ECCV 2012: 12th European Conference on Computer Vision, Florence, Italy, October 7-13, 2012, Proceedings, Part II 12},
  pages={474--487},
  year={2012},
  organization={Springer}
}
@article{zou2005regularization,
  title={Regularization and variable selection via the elastic net},
  author={Zou, Hui and Hastie, Trevor},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={67},
  number={2},
  pages={301--320},
  year={2005},
  publisher={Oxford University Press}
}
@article{tanveer2021large,
  title={Large-scale pinball twin support vector machines},
  author={Tanveer, M and Tiwari, Aruna and Choudhary, Rahul and Ganaie, MA},
  journal={Machine Learning},
  pages={1--24},
  year={2021},
  publisher={Springer}
}
@article{ganaie2022large,
  title={Large-scale fuzzy least squares twin {SVMs} for class imbalance learning},
  author={Ganaie, MA and Tanveer, M and Lin, Chin-Teng},
  journal={IEEE Transactions on Fuzzy Systems},
  volume={30},
  number={11},
  pages={4815--4827},
  year={2022},
  publisher={IEEE}
}

@article{richhariya2020reduced,
  title={A reduced universum twin support vector machine for class imbalance learning},
  author={Richhariya, Bharat and Tanveer, Muhammad},
  journal={Pattern Recognition},
  volume={102},
  pages={107150},
  year={2020},
  publisher={Elsevier}
}

@article{tang2020bearing,
  title={A bearing fault diagnosis method based on feature selection feedback network and improved {DS} evidence fusion},
  author={Tang, Xianghong and Gu, Xin and Wang, Jiachen and He, Qiang and Zhang, Fan and Lu, Jianguang},
  journal={IEEE Access},
  volume={8},
  pages={20523--20536},
  year={2020},
  publisher={IEEE}
}
@article{goldstein2014fast,
  title={Fast alternating direction optimization methods},
  author={Goldstein, Tom and O'Donoghue, Brendan and Setzer, Simon and Baraniuk, Richard},
  journal={SIAM Journal on Imaging Sciences},
  volume={7},
  number={3},
  pages={1588--1623},
  year={2014},
  publisher={SIAM}
}
@article{cai2010singular,
  title={A singular value thresholding algorithm for matrix completion},
  author={Cai, Jian-Feng and Cand{\`e}s, Emmanuel J and Shen, Zuowei},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={4},
  pages={1956--1982},
  year={2010},
  publisher={SIAM}
}
@article{tanveer2021sparse,
  title={Sparse support vector machine with pinball loss},
  author={Tanveer, Mohammad and Sharma, Sweta and Rastogi, Reshma and Anand, Pritam},
  journal={Transactions on Emerging Telecommunications Technologies},
  volume={32},
  number={2},
  pages={e3820},
  year={2021},
  publisher={Wiley Online Library}
}
@article{wu2007robust,
  title={Robust truncated hinge loss support vector machines},
  author={Wu, Yichao and Liu, Yufeng},
  journal={Journal of the American Statistical Association},
  volume={102},
  number={479},
  pages={974--983},
  year={2007},
  publisher={Taylor \& Francis}
}
@article{chen2013reduced,
  title={Reduced rank regression via adaptive nuclear norm penalization},
  author={Chen, Kun and Dong, Hongbo and Chan, Kung-Sik},
  journal={Biometrika},
  volume={100},
  number={4},
  pages={901--920},
  year={2013},
  publisher={Oxford University Press}
}
@article{liu2015truncated,
  title={A truncated nuclear norm regularization method based on weighted residual error for matrix completion},
  author={Liu, Qing and Lai, Zhihui and Zhou, Zongwei and Kuang, Fangjun and Jin, Zhong},
  journal={IEEE Transactions on Image Processing},
  volume={25},
  number={1},
  pages={316--330},
  year={2015},
  publisher={IEEE}
}
@article{jia2018bayesian,
  title={Bayesian inference for adaptive low rank and sparse matrix estimation},
  author={Jia, Xixi and Feng, Xiangchu and Wang, Weiwei and Xu, Chen and Zhang, Lei},
  journal={Neurocomputing},
  volume={291},
  pages={71--83},
  year={2018},
  publisher={Elsevier}
}
@article{dixit2020leveraging,
  title={Leveraging tacit knowledge for shipyard facility layout selection using fuzzy set theory},
  author={Dixit, Vijaya and Verma, Priyanka and Raj, Piyush},
  journal={Expert Systems with Applications},
  volume={158},
  pages={113423},
  year={2020},
  publisher={Elsevier}
}
@article{hong2016online,
  title={Online robust principal component analysis via truncated nuclear norm regularization},
  author={Hong, Bin and Wei, Long and Hu, Yao and Cai, Deng and He, Xiaofei},
  journal={Neurocomputing},
  volume={175},
  pages={216--222},
  year={2016},
  publisher={Elsevier}
}
@article{brooks2011support,
  title={Support vector machines with the ramp loss and the hard margin loss},
  author={Brooks, J Paul},
  journal={Operations research},
  volume={59},
  number={2},
  pages={467--479},
  year={2011},
  publisher={INFORMS}
}
@article{joachims2009cutting,
  title={Cutting-plane training of structural {SVM}s},
  author={Joachims, Thorsten and Finley, Thomas and Yu, Chun-Nam John},
  journal={Machine learning},
  volume={77},
  pages={27--59},
  year={2009},
  publisher={Springer}
}
@article{zhang2014multicategory,
  title={Multicategory angle-based large-margin classification},
  author={Zhang, Chong and Liu, Yufeng},
  journal={Biometrika},
  volume={101},
  number={3},
  pages={625--640},
  year={2014},
  publisher={Oxford University Press}
}
@article{sun2017angle,
  title={Angle-based multicategory distance-weighted {SVM}},
  author={Sun, Hui and Craig, Bruce A and Zhang, Lingsong},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={2981--3001},
  year={2017},
  publisher={JMLR. org}
}
@article{rosales2018mc2esvm,
  title={{MC2ESVM}: Multiclass classification based on cooperative evolution of support vector machines},
  author={Rosales-Perez, Alejandro and Garc{\'\i}a, Salvador and Terashima-Marin, Hugo and Coello, Carlos A Coello and Herrera, Francisco},
  journal={IEEE Computational Intelligence Magazine},
  volume={13},
  number={2},
  pages={18--29},
  year={2018},
  publisher={IEEE}
}
@inproceedings{bottou1994comparison,
  title={Comparison of classifier methods: a case study in handwritten digit recognition},
  author={Bottou, L{\'e}on and Cortes, Corinna and Denker, John S and Drucker, Harris and Guyon, Isabelle and Jackel, Larry D and LeCun, Yann and Muller, Urs A and Sackinger, Edward and Simard, Patrice and others},
  booktitle={Proceedings of the 12th IAPR International Conference on Pattern Recognition, Vol. 3-Conference C: Signal Processing (Cat. No. 94CH3440-5)},
  volume={2},
  pages={77--82},
  year={1994},
  organization={IEEE}
}
@article{uh1999pairwise,
  title={Pairwise classification and support vector machine},
  author={UH-G, KREISSEL},
  journal={Advances in kernel methods},
  year={1999}
}
@article{tao2020affinity,
  title={Affinity and class probability-based fuzzy support vector machine for imbalanced data sets},
  author={Tao, Xinmin and Li, Qing and Ren, Chao and Guo, Wenjie and He, Qing and Liu, Rui and Zou, Junrong},
  journal={Neural Networks},
  volume={122},
  pages={289--307},
  year={2020},
  publisher={Elsevier}
}
@article{mirjalili2016whale,
  title={The whale optimization algorithm},
  author={Mirjalili, Seyedali and Lewis, Andrew},
  journal={Advances in Engineering Software},
  volume={95},
  pages={51--67},
  year={2016},
  publisher={Elsevier}
}
@article{yu2018multisynchrosqueezing,
  title={Multisynchrosqueezing transform},
  author={Yu, Gang and Wang, Zhonghua and Zhao, Ping},
  journal={IEEE Transactions on Industrial Electronics},
  volume={66},
  number={7},
  pages={5441--5455},
  year={2018},
  publisher={IEEE}
}
@article{wang2015visual,
  title={Visual data denoising with a unified Schatten-$p$ norm and $l_q$ norm regularized principal component pursuit},
  author={Wang, Jing and Wang, Meng and Hu, Xuegang and Yan, Shuicheng},
  journal={Pattern Recognition},
  volume={48},
  number={10},
  pages={3135--3144},
  year={2015},
  publisher={Elsevier}
}
@article{huang2022overview,
  title={An overview on twin support vector regression},
  author={Huang, Huajuan and Wei, Xiuxi and Zhou, Yongquan},
  journal={Neurocomputing},
  volume={490},
  pages={80--92},
  year={2022},
  publisher={Elsevier}
}
@article{li2023intelligent,
  title={Intelligent fault diagnosis of bevel gearboxes using semi-supervised probability support matrix machine and infrared imaging},
  author={Li, Xin and Li, Yong and Yan, Ke and Shao, Haidong and Lin, Janet Jing},
  journal={Reliability Engineering \& System Safety},
  volume={230},
  pages={108921},
  year={2023},
  publisher={Elsevier}
}

@article{zhu2005semi,
  title={Semi-supervised learning literature survey},
  author={Zhu, Xiaojin Jerry},
  year={2005},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}
@article{bennett1998semi,
  title={Semi-supervised support vector machines},
  author={Bennett, Kristin and Demiriz, Ayhan},
  journal={Advances in Neural Information Processing Systems},
  volume={11},
  year={1998}
}
@inproceedings{zhang2005parallel,
  title={A parallel {SVM} training algorithm on large-scale classification problems},
  author={Zhang, Jian-Pei and Li, Zhong-Wei and Yang, Jing},
  booktitle={2005 International Conference on Machine Learning and Cybernetics},
  volume={3},
  pages={1637--1641},
  year={2005},
  organization={IEEE}
}
@article{vapnik2009new,
  title={A new learning paradigm: Learning using privileged information},
  author={Vapnik, Vladimir and Vashist, Akshay},
  journal={Neural Networks},
  volume={22},
  number={5-6},
  pages={544--557},
  year={2009},
  publisher={Elsevier}
}
@article{houthuys2018multi,
  title={Multi-view least squares support vector machines classification},
  author={Houthuys, Lynn and Langone, Rocco and Suykens, Johan AK},
  journal={Neurocomputing},
  volume={282},
  pages={78--88},
  year={2018},
  publisher={Elsevier}
}
@inproceedings{naeini2010stock,
  title={Stock market value prediction using neural networks},
  author={Naeini, Mahdi Pakdaman and Taremian, Hamidreza and Hashemi, Homa Baradaran},
  booktitle={2010 International Conference on Computer Information Systems and Industrial Management Applications (CISIM)},
  pages={132--136},
  year={2010},
  organization={IEEE}
}
@inproceedings{laurikkala2001improving,
  title={Improving identification of difficult small classes by balancing class distribution},
  author={Laurikkala, Jorma},
  booktitle={Artificial Intelligence in Medicine: 8th Conference on Artificial Intelligence in Medicine in Europe, AIME, Proceedings 8},
  pages={63--66},
  year={2001},
  organization={Springer}
}
@article{hart1968condensed,
  title={The condensed nearest neighbor rule (corresp.)},
  author={Hart, Peter},
  journal={IEEE Transactions on Information Theory},
  volume={14},
  number={3},
  pages={515--516},
  year={1968},
  publisher={Citeseer}
}
@article{chawla2002smote,
  title={{SMOTE}: synthetic minority over-sampling technique},
  author={Chawla, Nitesh V and Bowyer, Kevin W and Hall, Lawrence O and Kegelmeyer, W Philip},
  journal={Journal of Artificial Intelligence Research},
  volume={16},
  pages={321--357},
  year={2002}
}
@article{tanveer2022diagnosis,
  title={Diagnosis of schizophrenia: a comprehensive evaluation},
  author={Tanveer, Muhammad and Jangir, Jatin and Ganaie, MA and Beheshti, Iman and Tabish, M and Chhabra, Nikunj},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={27},
  number={3},
  pages={1185--1192},
  year={2022},
  publisher={IEEE}
}
@article{tanveer2020machine,
  title={Machine learning techniques for the diagnosis of Alzheimer’s disease: A review},
  author={Tanveer, Muhammad and Richhariya, Bharat and Khan, Riyaj Uddin and Rashid, Ashraf Haroon and Khanna, Pritee and Prasad, Mukesh and Lin, CT},
  journal={ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM)},
  volume={16},
  number={1s},
  pages={1--35},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{ma2019linex,
  title={{LINEX} support vector machine for large-scale classification},
  author={Ma, Yue and Zhang, Qin and Li, Dewei and Tian, Yingjie},
  journal={IEEE Access},
  volume={7},
  pages={70319--70331},
  year={2019},
  publisher={IEEE}
}
@article{tian2023kernel,
  title={Kernel methods with asymmetric and robust loss function},
  author={Tian, Yingjie and Zhao, Xiaoxi and Fu, Saiji},
  journal={Expert Systems with Applications},
  volume={213},
  pages={119236},
  year={2023},
  publisher={Elsevier}
}
@article{shen2017support,
  title={Support vector machine classifier with truncated pinball loss},
  author={Shen, Xin and Niu, Lingfeng and Qi, Zhiquan and Tian, Yingjie},
  journal={Pattern Recognition},
  volume={68},
  pages={199--210},
  year={2017},
  publisher={Elsevier}
}
@article{feng2016robust,
  title={Robust support vector machines for classification with nonconvex and smooth losses},
  author={Feng, Yunlong and Yang, Yuning and Huang, Xiaolin and Mehrkanoon, Siamak and Suykens, Johan AK},
  journal={Neural Computation},
  volume={28},
  number={6},
  pages={1217--1247},
  year={2016},
  publisher={MIT Press}
}
@article{das2010differential,
  title={Differential evolution: A survey of the state-of-the-art},
  author={Das, Swagatam and Suganthan, Ponnuthurai Nagaratnam},
  journal={IEEE Transactions on Evolutionary Computation},
  volume={15},
  number={1},
  pages={4--31},
  year={2010},
  publisher={IEEE}
}
@inproceedings{winters2007svm,
  title={{SVM} clustering},
  author={Winters-Hilt, Stephen and Merat, Sam},
  booktitle={BMC Bioinformatics},
  volume={8},
  number={7},
  pages={1--12},
  year={2007},
  organization={BioMed Central}
}
@article{mountrakis2011support,
  title={Support vector machines in remote sensing: A review},
  author={Mountrakis, Giorgos and Im, Jungho and Ogole, Caesar},
  journal={ISPRS Journal of Photogrammetry and Remote Sensing},
  volume={66},
  number={3},
  pages={247--259},
  year={2011},
  publisher={Elsevier}
}
@article{rezvani2023broad,
  title={A broad review on class imbalance learning techniques},
  author={Rezvani, Salim and Wang, Xizhao},
  journal={Applied Soft Computing},
  pages={110415},
  year={2023},
  publisher={Elsevier}
}
@book{lee2004first,
  title={First course on fuzzy theory and applications},
  author={Lee, Kwang Hyung},
  volume={27},
  year={2004},
  publisher={Springer Science \& Business Media}
}

@article{rezvani2019intuitionistic,
  title={Intuitionistic fuzzy twin support vector machines},
  author={Rezvani, Salim and Wang, Xizhao and Pourpanah, Farhad},
  journal={IEEE Transactions on Fuzzy Systems},
  volume={27},
  number={11},
  pages={2140--2151},
  year={2019},
  publisher={IEEE}
}
@article{richhariya2018eeg,
  title={{EEG} signal classification using universum support vector machine},
  author={Richhariya, Bharat and Tanveer, Muhammad},
  journal={Expert Systems with Applications},
  volume={106},
  pages={169--182},
  year={2018},
  publisher={Elsevier}
}
@article{ganaie2022brain,
  title={Brain age prediction with improved least squares twin SVR},
  author={Ganaie, MA and Tanveer, M and Beheshti, Iman},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={27},
  number={4},
  pages={1661--1669},
  year={2022},
  publisher={IEEE}
}
@article{bischof2021geometric,
  title={Geometric feature performance under downsampling for {EEG} classification tasks},
  author={Bischof, Bryan and Bunch, Eric},
  journal={arXiv preprint arXiv:2102.07669},
  year={2021}
}
@article{praline2007emergent,
  title={Emergent {EEG} in clinical practice},
  author={Praline, Julien and Grujic, J{\'e}l{\'e}na and Corcia, Philippe and Lucas, Brigitte and Hommet, Caroline and Autret, Alain and De Toffol, Bertrand},
  journal={Clinical Neurophysiology},
  volume={118},
  number={10},
  pages={2149--2155},
  year={2007},
  publisher={Elsevier}
}
@inproceedings{vaid2015eeg,
  title={{EEG} signal analysis for BCI interface: A review},
  author={Vaid, Swati and Singh, Preeti and Kaur, Chamandeep},
  booktitle={2015 Fifth International Conference on Advanced Computing \& Communication Technologies},
  pages={143--147},
  year={2015},
  organization={IEEE}
}
@phdthesis{pernestaal2009probabilistic,
  title={Probabilistic fault diagnosis with automotive applications},
  author={Pernest{\aa}l, Anna},
  year={2009},
  school={Link{\"o}ping University Electronic Press}
}
@inproceedings{pise2021comparative,
  title={Comparative analysis of various filtering techniques for denoising {EEG} signals},
  author={Pise, Anjali W and Rege, Priti P},
  booktitle={2021 6th International Conference for Convergence in Technology (I2CT)},
  pages={1--4},
  year={2021},
  organization={IEEE}
}
@article{ferdowsi2013online,
  title={An online outlier identification and removal scheme for improving fault detection performance},
  author={Ferdowsi, Hasan and Jagannathan, Sarangapani and Zawodniok, Maciej},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={25},
  number={5},
  pages={908--919},
  year={2013},
  publisher={IEEE}
}
@article{sekine1992fault,
  title={Fault diagnosis of power systems},
  author={Sekine, Yasuji and Akimoto, Yoshiakira and Kunugi, Masahiko and Fukui, Chihiro and Fukui, Shinta},
  journal={Proceedings of the IEEE},
  volume={80},
  number={5},
  pages={673--683},
  year={1992},
  publisher={IEEE}
}
@inproceedings{patton1990fault,
  title={Fault detection and diagnosis in aerospace systems using analytical redundancy},
  author={Patton, Ron J},
  booktitle={IEE Colloquium on Condition Monitoring and Fault Tolerance},
  pages={1--1},
  year={1990},
  organization={IET}
}
@article{yan2023review,
  title={A Review of Real-Time Fault Diagnosis Methods for Industrial Smart Manufacturing},
  author={Yan, Wenhao and Wang, Jing and Lu, Shan and Zhou, Meng and Peng, Xin},
  journal={Processes},
  volume={11},
  number={2},
  pages={369},
  year={2023},
  publisher={MDPI}
}

@inproceedings{sen2023review,
  title={A Review of the Filtering Techniques used in {EEG} Signal Processing},
  author={Sen, Dipanwita and Mishra, Bhupati Bhusan and Pattnaik, Prasant Kumar},
  booktitle={2023 7th International Conference on Trends in Electronics and Informatics (ICOEI)},
  pages={270--277},
  year={2023},
  organization={IEEE}
}

@article{devlaminck2011multisubject,
  title={Multisubject learning for common spatial patterns in motor-imagery {BCI}},
  author={Devlaminck, Dieter and Wyns, Bart and Grosse-Wentrup, Moritz and Otte, Georges and Santens, Patrick},
  journal={Computational Intelligence and Neuroscience},
  volume={2011},
  pages={8--8},
  year={2011},
  publisher={Hindawi Limited London, UK, United Kingdom}
}
@article{kuncheva2013pca,
  title={{PCA} feature extraction for change detection in multidimensional unlabeled data},
  author={Kuncheva, Ludmila I and Faithfull, William J},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={25},
  number={1},
  pages={69--80},
  year={2013},
  publisher={IEEE}
}
@article{shakshi2016brain,
  title={Brain wave classification and feature extraction of {EEG} signal by using {FFT} on lab view},
  author={Shakshi, Ramavtar Jaswal and Jaswal, R},
  journal={Int. Res. J. Eng. Technol},
  volume={3},
  pages={1208--1212},
  year={2016}
}
@article{vidaurre2009time,
  title={Time domain parameters as a feature for {EEG}-based brain--computer interfaces},
  author={Vidaurre, Carmen and Kr{\"a}mer, Nicole and Blankertz, Benjamin and Schl{\"o}gl, Alois},
  journal={Neural Networks},
  volume={22},
  number={9},
  pages={1313--1319},
  year={2009},
  publisher={Elsevier}
}
@book{hu2019eeg,
  title={{EEG} signal processing and feature extraction},
  author={Hu, Li and Zhang, Zhiguo},
  year={2019},
  publisher={Springer}
}

@article{usakli2010improvement,
  title={Improvement of {EEG} signal acquisition: An electrical aspect for state of the art of front end},
  author={Usakli, Ali Bulent and others},
  journal={Computational Intelligence and Neuroscience},
  volume={2010},
  year={2010},
  publisher={Hindawi}
}
@article{nicolas2012brain,
  title={Brain computer interfaces, a review},
  author={Nicolas-Alonso, Luis Fernando and Gomez-Gil, Jaime},
  journal={Sensors},
  volume={12},
  number={2},
  pages={1211--1279},
  year={2012},
  publisher={Molecular Diversity Preservation International (MDPI)}
}
@inproceedings{acharya2021multi,
  title={Multi-class emotion classification using {EEG} signals},
  author={Acharya, Divya and Jain, Riddhi and Panigrahi, Siba Smarak and Sahni, Rahul and Jain, Siddhi and Deshmukh, Sanika Prashant and Bhardwaj, Arpit},
  booktitle={Advanced Computing: 10th International Conference, IACC 2020, Panaji, Goa, India, December 5--6, 2020, Revised Selected Papers, Part I 10},
  pages={474--491},
  year={2021},
  organization={Springer}
}
@article{mumtaz2021review,
  title={Review of challenges associated with the {EEG} artifact removal methods},
  author={Mumtaz, Wajid and Rasheed, Suleman and Irfan, Alina},
  journal={Biomedical Signal Processing and Control},
  volume={68},
  pages={102741},
  year={2021},
  publisher={Elsevier}
}
@article{varbu2022past,
  title={Past, present, and future of {EEG}-based BCI applications},
  author={V{\"a}rbu, Kaido and Muhammad, Naveed and Muhammad, Yar},
  journal={Sensors},
  volume={22},
  number={9},
  pages={3331},
  year={2022},
  publisher={MDPI}
}
@article{srinivasan2007cognitive,
  title={Cognitive neuroscience of creativity: {EEG} based approaches},
  author={Srinivasan, Narayanan},
  journal={Methods},
  volume={42},
  number={1},
  pages={109--116},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{liu2019polsar,
  title={Polsar image classification based on polarimetric scattering coding and sparse support matrix machine},
  author={Liu, Xu and Jiao, Licheng and Zhang, Dan and Liu, Fang},
  booktitle={IGARSS 2019-2019 IEEE International Geoscience and Remote Sensing Symposium},
  pages={3181--3184},
  year={2019},
  organization={IEEE}
}
@inproceedings{iglovikov2018paediatric,
  title={Paediatric bone age assessment using deep convolutional neural networks},
  author={Iglovikov, Vladimir I and Rakhlin, Alexander and Kalinin, Alexandr A and Shvets, Alexey A},
  booktitle={Deep Learning in Medical Image Analysis and Multimodal Learning for Clinical Decision Support: 4th International Workshop, DLMIA 2018, and 8th International Workshop, ML-CDS 2018, Held in Conjunction with MICCAI 2018, Granada, Spain, September 20, 2018, Proceedings 4},
  pages={300--308},
  year={2018},
  organization={Springer}
}

@article{platt1998sequential,
  title={Sequential minimal optimization: A fast algorithm for training support vector machines},
  author={Platt, John},
  year={1998}
}
@article{keerthi2001improvements,
  title={Improvements to Platt's {SMO} algorithm for {SVM} classifier design},
  author={Keerthi, S. Sathiya and Shevade, Shirish Krishnaj and Bhattacharyya, Chiranjib and Murthy, Karuturi Radha Krishna},
  journal={Neural Computation},
  volume={13},
  number={3},
  pages={637--649},
  year={2001},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}
@article{cervantes2020comprehensive,
  title={A comprehensive survey on support vector machine classification: Applications, challenges and trends},
  author={Cervantes, Jair and Garcia-Lamont, Farid and Rodr{\'\i}guez-Mazahua, Lisbeth and Lopez, Asdrubal},
  journal={Neurocomputing},
  volume={408},
  pages={189--215},
  year={2020},
  publisher={Elsevier}
}
@article{suykens1999least,
  title={Least squares support vector machine classifiers},
  author={Suykens, Johan AK and Vandewalle, Joos},
  journal={Neural Processing Letters},
  volume={9},
  pages={293--300},
  year={1999},
  publisher={Springer}
}
@article{zhang2004wavelet,
  title={Wavelet support vector machine},
  author={Zhang, Li and Zhou, Weida and Jiao, Licheng},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
  volume={34},
  number={1},
  pages={34--39},
  year={2004},
  publisher={IEEE}
}

@article{zhang1992wavelet,
  title={Wavelet networks},
  author={Zhang, Qinghua and Benveniste, Albert},
  journal={IEEE Transactions on Neural Networks},
  volume={3},
  number={6},
  pages={889--898},
  year={1992},
  publisher={IEEE}
}

@inproceedings{franc2002multi,
  title={Multi-class support vector machine},
  author={Franc, Vojtech and Hlav{\'a}c, V{\'a}clav},
  booktitle={2002 International Conference on Pattern Recognition},
  volume={2},
  pages={236--239},
  year={2002},
  organization={IEEE}
}

@article{hullermeier2005fuzzy,
  title={Fuzzy methods in machine learning and data mining: Status and prospects},
  author={H{\"u}llermeier, Eyke},
  journal={Fuzzy Sets and Systems},
  volume={156},
  number={3},
  pages={387--406},
  year={2005},
  publisher={Elsevier}
}
@article{thakur2011synchrosqueezing,
  title={Synchrosqueezing-based recovery of instantaneous frequency from nonuniform samples},
  author={Thakur, Gaurav and Wu, Hau-Tieng},
  journal={SIAM Journal on Mathematical Analysis},
  volume={43},
  number={5},
  pages={2078--2095},
  year={2011},
  publisher={SIAM}
}
@article{weiss2016survey,
  title={A survey of transfer learning},
  author={Weiss, Karl and Khoshgoftaar, Taghi M and Wang, DingDing},
  journal={Journal of Big Data},
  volume={3},
  number={1},
  pages={1--40},
  year={2016},
  publisher={SpringerOpen}
}
@article{feng2022support,
  title={Support matrix machine with pinball loss for classification},
  author={Feng, Renxiu and Xu, Yitian},
  journal={Neural Computing and Applications},
  volume={34},
  number={21},
  pages={18643--18661},
  year={2022},
  publisher={Springer}
}

@article{fei2006one,
  title={One-shot learning of object categories},
  author={Fei-Fei, Li and Fergus, Robert and Perona, Pietro},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={28},
  number={4},
  pages={594--611},
  year={2006},
  publisher={IEEE}
}

@article{smola2004tutorial,
  title={A tutorial on support vector regression},
  author={Smola, Alex J and Sch{\"o}lkopf, Bernhard},
  journal={Statistics and Computing},
  volume={14},
  pages={199--222},
  year={2004},
  publisher={Springer}
}
@article{tang2019real,
  title={A real-time arrhythmia heartbeats classification algorithm using parallel delta modulations and rotated linear-kernel support vector machines},
  author={Tang, Xiaochen and Ma, Ziwei and Hu, Qisong and Tang, Wei},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={67},
  number={4},
  pages={978--986},
  year={2019},
  publisher={IEEE}
}

@article{derrac2015keel,
  title={{KEEL} data-mining software tool: Data set repository, integration of algorithms and experimental analysis framework},
  author={Derrac, J and Garcia, S and Sanchez, L and Herrera, F},
  journal={J. Mult. Valued Logic Soft Comput},
  volume={17},
  year={2015}
}

@article{saul2004overview,
  title={An overview of online learning},
  author={Saul Carliner},
  year={2004},
  publisher={Human Resource Development}
}

@article{majid2014prediction,
  title={Prediction of human breast and colon cancers from imbalanced data using nearest neighbor and support vector machines},
  author={Majid, Abdul and Ali, Safdar and Iqbal, Mubashar and Kausar, Nabeela},
  journal={Computer Methods and Programs in Biomedicine},
  volume={113},
  number={3},
  pages={792--808},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{tang2006fast,
  title={Fast and effective spam sender detection with granular {SVM} on highly imbalanced mail server behavior data},
  author={Tang, Yuchun and Krasser, Sven and Judge, Paul and Zhang, Yan-Qing},
  booktitle={2006 International Conference on Collaborative Computing: Networking, Applications and Worksharing},
  pages={1--6},
  year={2006},
  organization={IEEE}
}

@article{arshad2020estimating,
  title={On estimating the location parameter of the selected exponential population under the LINEX loss function},
  author={Arshad, Mohd and Abdalghani, Omer},
  year={2020}
}

@article{akhtar2023roboss,
  title={RoBoSS: A Robust, Bounded, Sparse, and Smooth Loss Function for Supervised Learning},
  author={Akhtar, Mushir and Tanveer, M and Arshad, Mohd},
  journal={arXiv preprint arXiv:2309.02250},
  year={2023}
}
